Evaluating the Ripple Effects of Knowledge Editing in Language Models

Modern language models capture a large body of factual knowledge. However, some facts can be incorrectly induced or become obsolete over time, resulting in factually incorrect generations. This has led to the development of various editing methods that allow updating facts encoded by the model. Evaluation of these methods has primarily focused on testing whether an individual fact has been successfully injected, and if similar predictions for other subjects have not changed. Here we argue that such evaluation is limited, since injecting one fact (e.g. ``Jack Depp is the son of Johnny Depp'') introduces a ``ripple effect'' in the form of additional facts that the model needs to update (e.g.``Jack Depp is the sibling of Lily-Rose Depp''). To address this issue, we propose a novel set of evaluation criteria that consider the implications of an edit on related facts. Using these criteria, we then construct RippleEdits, a diagnostic benchmark of 5K factual edits, capturing a variety of types of ripple effects. We evaluate prominent editing methods on RippleEdits, showing that current methods fail to introduce consistent changes in the model's knowledge. In addition, we find that a simple in-context editing baseline obtains the best scores on our benchmark, suggesting a promising research direction for model editing.

==> tables/results_filtering.tex <==


% \begin{table*}[t]
%     \centering
%     \footnotesize
%     \begin{tabular}{lllccrr}
%     & \textit{Relation} & \textit{Logical} & & & \textit{Subject} &   \\
%     & \textit{Specificity} & \textit{generalization} & \textit{Comp. I} & \textit{Comp. II} & \textit{Aliasing} & \textit{Forgetfulness} \\ \midrule
%         \gptxl{}
%          &$-$ &$-$ &$-$ &$-$ &$-$ &$-$  \\ \midrule
%          \gptj{}
%          &$-$ &$-$ &$-$ &$-$ &$-$ &$-$  \\ \midrule
%          \gptneo{} 
%          &$37.6$ &$75.3$ &$44.5$ &$81.3$ &$92.3$ &$95.0$   \\ \midrule
%          \llama{} 
%          &$-$ &$-$ &$-$ &$-$ &$-$ &$-$  \\ \midrule
%          \gptt{} 
%          &$-$ &$-$ &$-$ &$-$ &$-$ &$-$  \\
%          \bottomrule 
%     \end{tabular}
%     \caption{Averaged portion (in percentage) of queries from each of the tests, that have been considered during our evaluation, namely that their conditions have been met.}
% \label{table:filtered_tests_portion}
% \end{table*}

==> tacl2021_before_update_bib <==
% Use this file for citations not found in the ACL Anthology (contained in "anthology.bib").
@misc{gupta2023editing,
      title={Editing Commonsense Knowledge in GPT}, 
      author={Anshita Gupta and Debanjan Mondal and Akshay Krishna Sheshadri and Wenlong Zhao and Xiang Lorraine Li and Sarah Wiegreffe and Niket Tandon},
      year={2023},
      eprint={2305.14956},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{zhang-etal-2019-ernie,
    title = "{ERNIE}: Enhanced Language Representation with Informative Entities",
    author = "Zhang, Zhengyan  and
      Han, Xu  and
      Liu, Zhiyuan  and
      Jiang, Xin  and
      Sun, Maosong  and
      Liu, Qun",
    booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P19-1139",
    doi = "10.18653/v1/P19-1139",
    pages = "1441--1451",
    abstract = "Neural language representation models such as BERT pre-trained on large-scale corpora can well capture rich semantic patterns from plain text, and be fine-tuned to consistently improve the performance of various NLP tasks. However, the existing pre-trained language models rarely consider incorporating knowledge graphs (KGs), which can provide rich structured knowledge facts for better language understanding. We argue that informative entities in KGs can enhance language representation with external knowledge. In this paper, we utilize both large-scale textual corpora and KGs to train an enhanced language representation model (ERNIE), which can take full advantage of lexical, syntactic, and knowledge information simultaneously. The experimental results have demonstrated that ERNIE achieves significant improvements on various knowledge-driven tasks, and meanwhile is comparable with the state-of-the-art model BERT on other common NLP tasks. The code and datasets will be available in the future.",
}

@inproceedings{peters-etal-2019-knowledge,
    title = "Knowledge Enhanced Contextual Word Representations",
    author = "Peters, Matthew E.  and
      Neumann, Mark  and
      Logan, Robert  and
      Schwartz, Roy  and
      Joshi, Vidur  and
      Singh, Sameer  and
      Smith, Noah A.",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D19-1005",
    doi = "10.18653/v1/D19-1005",
    pages = "43--54",
    abstract = "Contextual word representations, typically trained on unstructured, unlabeled text, do not contain any explicit grounding to real world entities and are often unable to remember facts about those entities. We propose a general method to embed multiple knowledge bases (KBs) into large scale models, and thereby enhance their representations with structured, human-curated knowledge. For each KB, we first use an integrated entity linker to retrieve relevant entity embeddings, then update contextual word representations via a form of word-to-entity attention. In contrast to previous approaches, the entity linkers and self-supervised language modeling objective are jointly trained end-to-end in a multitask setting that combines a small amount of entity linking supervision with a large amount of raw text. After integrating WordNet and a subset of Wikipedia into BERT, the knowledge enhanced BERT (KnowBert) demonstrates improved perplexity, ability to recall facts as measured in a probing task and downstream performance on relationship extraction, entity typing, and word sense disambiguation. KnowBert{'}s runtime is comparable to BERT{'}s and it scales to large KBs.",
}

@inproceedings{
zhang2022greaselm,
title={Grease{LM}: Graph {REAS}oning Enhanced Language Models},
author={Xikun Zhang and Antoine Bosselut and Michihiro Yasunaga and Hongyu Ren and Percy Liang and Christopher D Manning and Jure Leskovec},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=41e9o6cQPj}
}

@misc{lewis2021retrievalaugmented,
      title={Retrieval-Augmented Generation for Knowledge-Intensive NLP Tasks}, 
      author={Patrick Lewis and Ethan Perez and Aleksandra Piktus and Fabio Petroni and Vladimir Karpukhin and Naman Goyal and Heinrich Küttler and Mike Lewis and Wen-tau Yih and Tim Rocktäschel and Sebastian Riedel and Douwe Kiela},
      year={2021},
      eprint={2005.11401},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{ijcai2021p552,
  title     = {Drop Redundant, Shrink Irrelevant: Selective Knowledge Injection for Language Pretraining},
  author    = {Zhang, Ningyu and Deng, Shumin and Cheng, Xu and Chen, Xi and Zhang, Yichi and Zhang, Wei and Chen, Huajun},
  booktitle = {Proceedings of the Thirtieth International Joint Conference on
               Artificial Intelligence, {IJCAI-21}},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},
  editor    = {Zhi-Hua Zhou},
  pages     = {4007--4014},
  year      = {2021},
  month     = {8},
  note      = {Main Track},
  doi       = {10.24963/ijcai.2021/552},
  url       = {https://doi.org/10.24963/ijcai.2021/552},
}


@misc{wang2020kadapter,
      title={K-Adapter: Infusing Knowledge into Pre-Trained Models with Adapters}, 
      author={Ruize Wang and Duyu Tang and Nan Duan and Zhongyu Wei and Xuanjing Huang and Jianshu ji and Guihong Cao and Daxin Jiang and Ming Zhou},
      year={2020},
      eprint={2002.01808},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{yao2022kformer,
      title={Kformer: Knowledge Injection in Transformer Feed-Forward Layers}, 
      author={Yunzhi Yao and Shaohan Huang and Li Dong and Furu Wei and Huajun Chen and Ningyu Zhang},
      year={2022},
      eprint={2201.05742},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{hernandez2023inspecting,
      title={Inspecting and Editing Knowledge Representations in Language Models}, 
      author={Evan Hernandez and Belinda Z. Li and Jacob Andreas},
      year={2023},
      eprint={2304.00740},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}


@misc{jang2023temporalwiki,
      title={TemporalWiki: A Lifelong Benchmark for Training and Evaluating Ever-Evolving Language Models}, 
      author={Joel Jang and Seonghyeon Ye and Changho Lee and Sohee Yang and Joongbo Shin and Janghoon Han and Gyeonghun Kim and Minjoon Seo},
      year={2023},
      eprint={2204.14211},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{dai-etal-2022-knowledge,
    title = "Knowledge Neurons in Pretrained Transformers",
    author = "Dai, Damai  and
      Dong, Li  and
      Hao, Yaru  and
      Sui, Zhifang  and
      Chang, Baobao  and
      Wei, Furu",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.581",
    doi = "10.18653/v1/2022.acl-long.581",
    pages = "8493--8502",
    abstract = "Large-scale pretrained language models are surprisingly good at recalling factual knowledge presented in the training corpus. In this paper, we present preliminary studies on how factual knowledge is stored in pretrained Transformers by introducing the concept of knowledge neurons. Specifically, we examine the fill-in-the-blank cloze task for BERT. Given a relational fact, we propose a knowledge attribution method to identify the neurons that express the fact. We find that the activation of such knowledge neurons is positively correlated to the expression of their corresponding facts. In our case studies, we attempt to leverage knowledge neurons to edit (such as update, and erase) specific factual knowledge without fine-tuning. Our results shed light on understanding the storage of knowledge within pretrained Transformers.",
}

@inproceedings{geva-etal-2021-transformer,
    title = "Transformer Feed-Forward Layers Are Key-Value Memories",
    author = "Geva, Mor  and
      Schuster, Roei  and
      Berant, Jonathan  and
      Levy, Omer",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.446",
    doi = "10.18653/v1/2021.emnlp-main.446",
    pages = "5484--5495",
    abstract = "Feed-forward layers constitute two-thirds of a transformer model{'}s parameters, yet their role in the network remains under-explored. We show that feed-forward layers in transformer-based language models operate as key-value memories, where each key correlates with textual patterns in the training examples, and each value induces a distribution over the output vocabulary. Our experiments show that the learned patterns are human-interpretable, and that lower layers tend to capture shallow patterns, while upper layers learn more semantic ones. The values complement the keys{'} input patterns by inducing output distributions that concentrate probability mass on tokens likely to appear immediately after each pattern, particularly in the upper layers. Finally, we demonstrate that the output of a feed-forward layer is a composition of its memories, which is subsequently refined throughout the model{'}s layers via residual connections to produce the final output distribution.",
}

@inproceedings{roberts-etal-2020-much,
    title = "How Much Knowledge Can You Pack Into the Parameters of a Language Model?",
    author = "Roberts, Adam  and
      Raffel, Colin  and
      Shazeer, Noam",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.437",
    doi = "10.18653/v1/2020.emnlp-main.437",
    pages = "5418--5426",
    abstract = "It has recently been observed that neural language models trained on unstructured text can implicitly store and retrieve knowledge using natural language queries. In this short paper, we measure the practical utility of this approach by fine-tuning pre-trained models to answer questions without access to any external context or knowledge. We show that this approach scales with model size and performs competitively with open-domain systems that explicitly retrieve answers from an external knowledge source when answering questions. To facilitate reproducibility and future work, we release our code and trained models.",
}

@misc{yao2023editing,
      title={Editing Large Language Models: Problems, Methods, and Opportunities}, 
      author={Yunzhi Yao and Peng Wang and Bozhong Tian and Siyuan Cheng and Zhoubo Li and Shumin Deng and Huajun Chen and Ningyu Zhang},
      year={2023},
      eprint={2305.13172},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{zhong2023mquake,
      title={MQuAKE: Assessing Knowledge Editing in Language Models via Multi-Hop Questions}, 
      author={Zexuan Zhong and Zhengxuan Wu and Christopher D. Manning and Christopher Potts and Danqi Chen},
      year={2023},
      eprint={2305.14795},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{hoelscherobermaier2023detecting,
      title={Detecting Edit Failures In Large Language Models: An Improved Specificity Benchmark}, 
      author={Jason Hoelscher-Obermaier and Julia Persson and Esben Kran and Ioannis Konstas and Fazl Barez},
      year={2023},
      eprint={2305.17553},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{onoe2023lms,
      title={Can LMs Learn New Entities from Descriptions? Challenges in Propagating Injected Knowledge}, 
      author={Yasumasa Onoe and Michael J. Q. Zhang and Shankar Padmanabhan and Greg Durrett and Eunsol Choi},
      year={2023},
      eprint={2305.01651},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{mitchell2022memorybased,
      title={Memory-Based Model Editing at Scale}, 
      author={Eric Mitchell and Charles Lin and Antoine Bosselut and Christopher D. Manning and Chelsea Finn},
      year={2022},
      eprint={2206.06520},
      archivePrefix={arXiv},
      primaryClass={cs.AI}
}

@misc{mitchell2022fast,
      title={Fast Model Editing at Scale}, 
      author={Eric Mitchell and Charles Lin and Antoine Bosselut and Chelsea Finn and Christopher D. Manning},
      year={2022},
      eprint={2110.11309},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{meng2023locating,
      title={Locating and Editing Factual Associations in GPT}, 
      author={Kevin Meng and David Bau and Alex Andonian and Yonatan Belinkov},
      year={2023},
      eprint={2202.05262},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{de-cao-etal-2021-editing,
    title = "Editing Factual Knowledge in Language Models",
    author = "De Cao, Nicola  and
      Aziz, Wilker  and
      Titov, Ivan",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.522",
    doi = "10.18653/v1/2021.emnlp-main.522",
    pages = "6491--6506",
    abstract = "The factual knowledge acquired during pre-training and stored in the parameters of Language Models (LMs) can be useful in downstream tasks (e.g., question answering or textual inference). However, some facts can be incorrectly induced or become obsolete over time. We present KnowledgeEditor, a method which can be used to edit this knowledge and, thus, fix {`}bugs{'} or unexpected predictions without the need for expensive re-training or fine-tuning. Besides being computationally efficient, KnowledgeEditordoes not require any modifications in LM pre-training (e.g., the use of meta-learning). In our approach, we train a hyper-network with constrained optimization to modify a fact without affecting the rest of the knowledge; the trained hyper-network is then used to predict the weight update at test time. We show KnowledgeEditor{'}s efficacy with two popular architectures and knowledge-intensive tasks: i) a BERT model fine-tuned for fact-checking, and ii) a sequence-to-sequence BART model for question answering. With our method, changing a prediction on the specific wording of a query tends to result in a consistent change in predictions also for its paraphrases. We show that this can be further encouraged by exploiting (e.g., automatically-generated) paraphrases during training. Interestingly, our hyper-network can be regarded as a {`}probe{'} revealing which components need to be changed to manipulate factual knowledge; our analysis shows that the updates tend to be concentrated on a small subset of components. Source code available at https://github.com/nicola-decao/KnowledgeEditor",
}

@inproceedings{levy-etal-2017-zero,
    title = "Zero-Shot Relation Extraction via Reading Comprehension",
    author = "Levy, Omer  and
      Seo, Minjoon  and
      Choi, Eunsol  and
      Zettlemoyer, Luke",
    booktitle = "Proceedings of the 21st Conference on Computational Natural Language Learning ({C}o{NLL} 2017)",
    month = aug,
    year = "2017",
    address = "Vancouver, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/K17-1034",
    doi = "10.18653/v1/K17-1034",
    pages = "333--342",
    abstract = "We show that relation extraction can be reduced to answering simple reading comprehension questions, by associating one or more natural-language questions with each relation slot. This reduction has several advantages: we can (1) learn relation-extraction models by extending recent neural reading-comprehension techniques, (2) build very large training sets for those models by combining relation-specific crowd-sourced questions with distant supervision, and even (3) do zero-shot learning by extracting new relation types that are only specified at test-time, for which we have no labeled training examples. Experiments on a Wikipedia slot-filling task demonstrate that the approach can generalize to new questions for known relation types with high accuracy, and that zero-shot generalization to unseen relation types is possible, at lower accuracy levels, setting the bar for future work on this task.",
}

@inproceedings{cohen-etal-2023-crawling,
    title = "Crawling The Internal Knowledge-Base of Language Models",
    author = "Cohen, Roi  and
      Geva, Mor  and
      Berant, Jonathan  and
      Globerson, Amir",
    booktitle = "Findings of the Association for Computational Linguistics: EACL 2023",
    month = may,
    year = "2023",
    address = "Dubrovnik, Croatia",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2023.findings-eacl.139",
    pages = "1856--1869",
    abstract = "Language models are trained on large volumes of text, and as a result their parameters might contain a significant body of factual knowledge. Any downstream task performed by these models implicitly builds on these facts, and thus it is highly desirable to have means for representing this body of knowledge in an interpretable way. However, there is currently no mechanism for such a representation.Here, we propose to address this goal by extracting a knowledge-graph of facts from a given language model. We describe a procedure for {``}crawling{''} the internal knowledge-base of a language model. Specifically, given a seed entity, we expand a knowledge-graph around it. The crawling procedure is decomposed into sub-tasks, realized through specially designed prompts that control for both precision (i.e., that no wrong facts are generated) and recall (i.e., the number of facts generated). We evaluate our approach on graphs crawled starting from dozens of seed entities, and show it yields high precision graphs (82-92{\%}), while emitting a reasonable number of facts per entity.",
}

@misc{bommasani2022opportunities,
      title={On the Opportunities and Risks of Foundation Models}, 
      author={Rishi Bommasani and Drew A. Hudson and Ehsan Adeli and Russ Altman and Simran Arora and Sydney von Arx and Michael S. Bernstein and Jeannette Bohg and Antoine Bosselut and Emma Brunskill and Erik Brynjolfsson and Shyamal Buch and Dallas Card and Rodrigo Castellon and Niladri Chatterji and Annie Chen and Kathleen Creel and Jared Quincy Davis and Dora Demszky and Chris Donahue and Moussa Doumbouya and Esin Durmus and Stefano Ermon and John Etchemendy and Kawin Ethayarajh and Li Fei-Fei and Chelsea Finn and Trevor Gale and Lauren Gillespie and Karan Goel and Noah Goodman and Shelby Grossman and Neel Guha and Tatsunori Hashimoto and Peter Henderson and John Hewitt and Daniel E. Ho and Jenny Hong and Kyle Hsu and Jing Huang and Thomas Icard and Saahil Jain and Dan Jurafsky and Pratyusha Kalluri and Siddharth Karamcheti and Geoff Keeling and Fereshte Khani and Omar Khattab and Pang Wei Koh and Mark Krass and Ranjay Krishna and Rohith Kuditipudi and Ananya Kumar and Faisal Ladhak and Mina Lee and Tony Lee and Jure Leskovec and Isabelle Levent and Xiang Lisa Li and Xuechen Li and Tengyu Ma and Ali Malik and Christopher D. Manning and Suvir Mirchandani and Eric Mitchell and Zanele Munyikwa and Suraj Nair and Avanika Narayan and Deepak Narayanan and Ben Newman and Allen Nie and Juan Carlos Niebles and Hamed Nilforoshan and Julian Nyarko and Giray Ogut and Laurel Orr and Isabel Papadimitriou and Joon Sung Park and Chris Piech and Eva Portelance and Christopher Potts and Aditi Raghunathan and Rob Reich and Hongyu Ren and Frieda Rong and Yusuf Roohani and Camilo Ruiz and Jack Ryan and Christopher Ré and Dorsa Sadigh and Shiori Sagawa and Keshav Santhanam and Andy Shih and Krishnan Srinivasan and Alex Tamkin and Rohan Taori and Armin W. Thomas and Florian Tramèr and Rose E. Wang and William Wang and Bohan Wu and Jiajun Wu and Yuhuai Wu and Sang Michael Xie and Michihiro Yasunaga and Jiaxuan You and Matei Zaharia and Michael Zhang and Tianyi Zhang and Xikun Zhang and Yuhui Zhang and Lucia Zheng and Kaitlyn Zhou and Percy Liang},
      year={2022},
      eprint={2108.07258},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{chowdhery2022palm,
      title={PaLM: Scaling Language Modeling with Pathways}, 
      author={Aakanksha Chowdhery and Sharan Narang and Jacob Devlin and Maarten Bosma and Gaurav Mishra and Adam Roberts and Paul Barham and Hyung Won Chung and Charles Sutton and Sebastian Gehrmann and Parker Schuh and Kensen Shi and Sasha Tsvyashchenko and Joshua Maynez and Abhishek Rao and Parker Barnes and Yi Tay and Noam Shazeer and Vinodkumar Prabhakaran and Emily Reif and Nan Du and Ben Hutchinson and Reiner Pope and James Bradbury and Jacob Austin and Michael Isard and Guy Gur-Ari and Pengcheng Yin and Toju Duke and Anselm Levskaya and Sanjay Ghemawat and Sunipa Dev and Henryk Michalewski and Xavier Garcia and Vedant Misra and Kevin Robinson and Liam Fedus and Denny Zhou and Daphne Ippolito and David Luan and Hyeontaek Lim and Barret Zoph and Alexander Spiridonov and Ryan Sepassi and David Dohan and Shivani Agrawal and Mark Omernick and Andrew M. Dai and Thanumalayan Sankaranarayana Pillai and Marie Pellat and Aitor Lewkowycz and Erica Moreira and Rewon Child and Oleksandr Polozov and Katherine Lee and Zongwei Zhou and Xuezhi Wang and Brennan Saeta and Mark Diaz and Orhan Firat and Michele Catasta and Jason Wei and Kathy Meier-Hellstern and Douglas Eck and Jeff Dean and Slav Petrov and Noah Fiedel},
      year={2022},
      eprint={2204.02311},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{NEURIPS2020_1457c0d6,
 author = {Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel and Wu, Jeffrey and Winter, Clemens and Hesse, Chris and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M.F. Balcan and H. Lin},
 pages = {1877--1901},
 publisher = {Curran Associates, Inc.},
 title = {Language Models are Few-Shot Learners},
 url = {https://proceedings.neurips.cc/paper_files/paper/2020/file/1457c0d6bfcb4967418bfb8ac142f64a-Paper.pdf},
 volume = {33},
 year = {2020}
}


@article{petroni2019language,
  title={Language models as knowledge bases?},
  author={Petroni, Fabio and Rockt{\"a}schel, Tim and Lewis, Patrick and Bakhtin, Anton and Wu, Yuxiang and Miller, Alexander H and Riedel, Sebastian},
  journal={arXiv preprint arXiv:1909.01066},
  year={2019}
}

@article{roberts2020much,
  title={How much knowledge can you pack into the parameters of a language model?},
  author={Roberts, Adam and Raffel, Colin and Shazeer, Noam},
  journal={arXiv preprint arXiv:2002.08910},
  year={2020}
}

@article{shin2020autoprompt,
  title={Autoprompt: Eliciting knowledge from language models with automatically generated prompts},
  author={Shin, Taylor and Razeghi, Yasaman and Logan IV, Robert L and Wallace, Eric and Singh, Sameer},
  journal={arXiv preprint arXiv:2010.15980},
  year={2020}
}

@article{elazar2021measuring,
  title={Measuring and improving consistency in pretrained language models},
  author={Elazar, Yanai and Kassner, Nora and Ravfogel, Shauli and Ravichander, Abhilasha and Hovy, Eduard and Sch{\"u}tze, Hinrich and Goldberg, Yoav},
  journal={Transactions of the Association for Computational Linguistics},
  volume={9},
  pages={1012--1031},
  year={2021},
  publisher={MIT Press}
}

@article{razniewski2021language,
  title={Language models as or for knowledge bases},
  author={Razniewski, Simon and Yates, Andrew and Kassner, Nora and Weikum, Gerhard},
  journal={arXiv preprint arXiv:2110.04888},
  year={2021}
}

@article{heinzerling2020language,
  title={Language models as knowledge bases: On entity representations, storage capacity, and paraphrased queries},
  author={Heinzerling, Benjamin and Inui, Kentaro},
  journal={arXiv preprint arXiv:2008.09036},
  year={2020}
}

@article{kadavath2022language,
  title={Language models (mostly) know what they know},
  author={Kadavath, Saurav and Conerly, Tom and Askell, Amanda and Henighan, Tom and Drain, Dawn and Perez, Ethan and Schiefer, Nicholas and Dodds, Zac Hatfield and DasSarma, Nova and Tran-Johnson, Eli and others},
  journal={arXiv preprint arXiv:2207.05221},
  year={2022}
}

@article{cohen2023crawling,
  title={Crawling the Internal Knowledge-Base of Language Models},
  author={Cohen, Roi and Geva, Mor and Berant, Jonathan and Globerson, Amir},
  journal={arXiv preprint arXiv:2301.12810},
  year={2023}
}

@article{dhingra2022time,
  title={Time-aware language models as temporal knowledge bases},
  author={Dhingra, Bhuwan and Cole, Jeremy R and Eisenschlos, Julian Martin and Gillick, Daniel and Eisenstein, Jacob and Cohen, William W},
  journal={Transactions of the Association for Computational Linguistics},
  volume={10},
  pages={257--273},
  year={2022},
  publisher={MIT Press}
}

@article{lazaridou2021mind,
  title={Mind the gap: Assessing temporal generalization in neural language models},
  author={Lazaridou, Angeliki and Kuncoro, Adhi and Gribovskaya, Elena and Agrawal, Devang and Liska, Adam and Terzi, Tayfun and Gimenez, Mai and de Masson d'Autume, Cyprien and Kocisky, Tomas and Ruder, Sebastian and others},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={29348--29363},
  year={2021}
}

@article{jang2021towards,
  title={Towards continual knowledge learning of language models},
  author={Jang, Joel and Ye, Seonghyeon and Yang, Sohee and Shin, Joongbo and Han, Janghoon and Kim, Gyeonghun and Choi, Stanley Jungkyu and Seo, Minjoon},
  journal={arXiv preprint arXiv:2110.03215},
  year={2021}
}

@article{meng2022locating,
  title={Locating and editing factual associations in GPT},
  author={Meng, Kevin and Bau, David and Andonian, Alex and Belinkov, Yonatan},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={17359--17372},
  year={2022}
}

@article{mitchell2021fast,
  title={Fast model editing at scale},
  author={Mitchell, Eric and Lin, Charles and Bosselut, Antoine and Finn, Chelsea and Manning, Christopher D},
  journal={arXiv preprint arXiv:2110.11309},
  year={2021}
}

@article{meng2022mass,
  title={Mass-editing memory in a transformer},
  author={Meng, Kevin and Sharma, Arnab Sen and Andonian, Alex and Belinkov, Yonatan and Bau, David},
  journal={arXiv preprint arXiv:2210.07229},
  year={2022}
}

@article{hernandez2023measuring,
  title={Measuring and Manipulating Knowledge Representations in Language Models},
  author={Hernandez, Evan and Li, Belinda Z and Andreas, Jacob},
  journal={arXiv preprint arXiv:2304.00740},
  year={2023}
}

@article{si2022prompting,
  title={Prompting gpt-3 to be reliable},
  author={Si, Chenglei and Gan, Zhe and Yang, Zhengyuan and Wang, Shuohang and Wang, Jianfeng and Boyd-Graber, Jordan and Wang, Lijuan},
  journal={arXiv preprint arXiv:2210.09150},
  year={2022}
}

@article{radford2019language,
  title={Language models are unsupervised multitask learners},
  author={Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya and others},
  journal={OpenAI blog},
  volume={1},
  number={8},
  pages={9},
  year={2019}
}

@article{chen2021evaluating,
  title={Evaluating large language models trained on code},
  author={Chen, Mark and Tworek, Jerry and Jun, Heewoo and Yuan, Qiming and Pinto, Henrique Ponde de Oliveira and Kaplan, Jared and Edwards, Harri and Burda, Yuri and Joseph, Nicholas and Brockman, Greg and others},
  journal={arXiv preprint arXiv:2107.03374},
  year={2021}
}

@article{black2022gpt,
  title={Gpt-neox-20b: An open-source autoregressive language model},
  author={Black, Sid and Biderman, Stella and Hallahan, Eric and Anthony, Quentin and Gao, Leo and Golding, Laurence and He, Horace and Leahy, Connor and McDonell, Kyle and Phang, Jason and others},
  journal={arXiv preprint arXiv:2204.06745},
  year={2022}
}

@article{touvron2023llama,
  title={Llama: Open and efficient foundation language models},
  author={Touvron, Hugo and Lavril, Thibaut and Izacard, Gautier and Martinet, Xavier and Lachaux, Marie-Anne and Lacroix, Timoth{\'e}e and Rozi{\`e}re, Baptiste and Goyal, Naman and Hambro, Eric and Azhar, Faisal and others},
  journal={arXiv preprint arXiv:2302.13971},
  year={2023}
}

@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}

@misc{openai2023gpt4,
      title={GPT-4 Technical Report}, 
      author={OpenAI},
      year={2023},
      eprint={2303.08774},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{mallen-etal-2023-trust,
    title = "When Not to Trust Language Models: Investigating Effectiveness of Parametric and Non-Parametric Memories",
    author = "Mallen, Alex  and
      Asai, Akari  and
      Zhong, Victor  and
      Das, Rajarshi  and
      Khashabi, Daniel  and
      Hajishirzi, Hannaneh",
    booktitle = "Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2023",
    address = "Toronto, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2023.acl-long.546",
    pages = "9802--9822"
}
